Evaluation of X-ray/EUV Nanolithography Facility at AS Through Wavefront Propagation Simulations

Synchrotron light sources can provide the required spatial coherence, stability and control that is required to support the development of advanced lithography at the extreme ultraviolet and soft X-ray wavelengths that are relevant to current and future fabricating technologies. Here we present an evaluation of the optical performance of the soft X-ray (SXR) beamline of the Australian Synchrotron (AS) and its suitability for developing interference lithography using radiation in the 91.8 eV (13.5 nm) to 300 eV (4.13 nm) range. A comprehensive physical optics model of the APPLE-II undulator source and SXR beamline was constructed to simulate the properties of the illumination at the proposed location of a photomask, as a function of photon energy, collimation, and monochromator parameters. The model is validated using a combination of experimental measurements of the photon intensity distribution of the undulator harmonics. We show that the undulator harmonics intensity ratio can be accurately measured using an imaging detector and controlled using beamline optics. Finally, we evaluate photomask geometric constraints and achievable performance for the limiting case of fully spatially coherent illumination.

==> beamlineGeometry.tex <==
% \singlecolumn
\begin{table}
% \begin{multicols}{1}
\caption{The typical geometry of the optical elements used in the model of the beamline and IL optics. The defining characteristic for a mirror is given as the major radius, \textit{R}, and minor radius, $\rho$. The defining characteristic for a grating is the periodicity, and for a mask the grating size, $G$. Aperture sizes shown were used for all simulations and measurements shown in this work unless stated otherwise.}
% \end{multicols}
\resizebox{\textwidth}{!}{\begin{tabular}{lrrrrrr}
\hline
\textbf{Element Name}     & \textbf{\begin{tabular}[c]{@{}r@{}}Element\\ Type\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}Propagation\\ Distance [m]\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}Distance from\\ Source [m]\end{tabular}} & \textbf{Dimensions [mm]}   & \textbf{\begin{tabular}[c]{@{}r@{}}Defining\\ Characteristics\end{tabular}} & \textbf{\begin{tabular}[c]{@{}r@{}}Incident\\ Angle [$^o$]\end{tabular}} \\ \hline
White Beam Slits          & Aperture                                                        & 14.30                                                                 & 14.30                                                                 & 4 $\times$ 3       & N/A                                                                         & 90                                                            \\
Toroidal Mirror           & Mirror                                                          & 0.82                                                                 & 15.12                                                                 & 420 $\times$ 30    & \begin{tabular}[c]{@{}r@{}}R = 6668 m\\ $\rho$ = 5.262 m\end{tabular}    & 1                                                             \\
Planar Mirror             & Mirror                                                          & 3.38                                                                  & 18.50                                                                 & 460 $\times$ 50    & N/A                                                                         & 2                                                             \\
Grating                   & Grating                                                         & 0.20                                                                  & 18.70                                                                 & 150 $\times$ 20    & 250 lines/mm                                                                & 1.173                                                        \\
Exit Aperture             & Aperture                                                        & 1.00                                                                  & 19.70                                                                 & 10 $\times$ 20     & N/A                                                                         & 90                                                            \\
Cylindrical Mirror        & Mirror                                                          & 0.60                                                                  & 20.30                                                                 & 240 $\times$ 40    & \begin{tabular}[c]{@{}r@{}}R = 100 km\\ $\rho$ = 0.2443 m\end{tabular}      & 1.5                                                           \\
Secondary Source Aperture & Aperture                                                        & 6.50                                                                  & 26.80                                                                 & 0.025 $\times$ 0.025   & N/A                                                                         & 90                                                            \\
Grating Mask              & Mask                                                            & 9.50                                                                  & 36.30                                                                 & 0.15 $\times$ 0.15 & \begin{tabular}[c]{@{}r@{}}$G$ = 50 \textmu m\end{tabular}  & 90                                                            \\ \hline
\end{tabular}}
\label{table:beamline}
\end{table}

==> storageRing.tex <==
\begin{table}
\caption{Key values for the Australian Synchrotron storage ring. Parameters obtained from \cite{wootton_observation_2012}}
\resizebox{\columnwidth}{!}
{\begin{tabular}{0.9\textwidth}%{llr}
\hline
             & Parameter                & Value        \\ \hline
$E_0$        & Beam Energy        & 3.01 GeV         \\
$I_0$        & Current               & 0.2 A         \\
$\sigma_E$   & RMS Energy Spread       & 0.1021 $\%$   \\
$\epsilon_x$ & Horizontal Emittance   & 10 nm rad   \\
$\epsilon_y$ & Vertical Emittance  & 0.009 nm rad  \\
$\beta_x$    & Horizontal Beta Function & 9 m          \\
$\beta_y$    & Vertical Beta Function  & 3 m          \\ \hline
\end{tabular}}
\label{table:storageRing}
\end{table}


%       Table 1: The citations for the data presented in this Table are: [9] a conference paper, [10] missing any journal information, and [11] a fact sheet. Suggest replacing these with primary journal references such as: Wootton, et al. Phys. Rev. Lett. 109, 194801 (2012): http://dx.doi.org/10.1103/PhysRevLett.109.194801
%       Tables 1-2: make sure that the set of parameters used for the source are self-consistent and complete, so that someone else using SRW could repeat the setup.

==> undulator.tex <==
\begin{table}
\caption{Key values for the APPLE-II undulator used for the SXR beamline at the Australian Synchrotron. $K_u$, which determines $B_u$, was adjusted to produce a fundamental harmonic at 184.76 eV. Other values obtained from Ref. \cite{wootton_observation_2012}}
\resizebox{\columnwidth}{!}{\begin{tabular}{llr}
\hline
            & Parameter                   & Value        \\ \hline
$L_u$       & Undulator Length           & 1.875 m     \\
$\lambda_u$ & Undulator Period Length     & 75 mm       \\
$N_u$       & Number of Undulator Periods & 25              \\
$B_u$       & Peak Magnetic Field         & 0.4611 T         \\
$K_u$       & Deflection Parameter        & 3.230           \\ \hline
\end{tabular}}
\label{table:undulator}
\end{table}
